Optimally balancing exploration and exploitation to automate multi-fidelity statistical estimation

Multi-fidelity methods that use an ensemble of models to compute a Monte Carlo estimator of the expectation of a high-fidelity model can significantly reduce computational costs compared to single-model approaches. These methods use oracle statistics, specifically the covariance between models, to optimally allocate samples to each model in the ensemble. However, in practice, the oracle statistics are estimated using additional model evaluations, whose computational cost and induced error are typically ignored. To address this issue, this paper proposes an adaptive algorithm to optimally balance the resources between oracle statistics estimation and final multi-fidelity estimator construction, leveraging ideas from multilevel best linear unbiased estimators in Schaden and Ullmann (2020) and a bandit-learning procedure in Xu et al. (2022). Under mild assumptions, we demonstrate that the multi-fidelity estimator produced by the proposed algorithm exhibits mean-squared error commensurate with that of the best linear unbiased estimator under the optimal allocation computed with oracle statistics. Our theoretical findings are supported by detailed numerical experiments, including a parametric elliptic PDE and an ice-sheet mass-change modeling problem.

==> tmp_main_header.tex <==
\title{Optimally balancing exploration and exploitation to automate multi-fidelity statistical estimation\thanks{Submitted to the editors on \today.
\funding{Dixon and Jakeman were supported by the US Department of Energy’s Office of Advanced Scientific Computing Research program. Gorodetsky was supported by the National Nuclear Security Administration’s Advanced Simulation and Computing (ASC) program. Narayan was supported by AFOSR FA9550-20-1-0338 and AFOSR FA9550-23-1-0749. Xu was supported by the University of Kentucky for the start-up funding and the AMS-Simons Travel grant (No.3048116562). Sandia National Laboratories is a multi-mission laboratory managed and operated by National Technology \& Engineering Solutions of Sandia, LLC (NTESS), a wholly owned subsidiary of Honeywell International Inc., for the U.S. Department of Energy’s National Nuclear Security Administration (DOE/NNSA) under contract DE-NA0003525. This written work is authored by an employee of NTESS. The employee, not NTESS, owns the right, title, and interest in and to the written work and is responsible for its contents. Any subjective views or opinions that might be expressed in the written work do not necessarily represent the views of the U.S. Government. The publisher acknowledges that the U.S. Government retains a non-exclusive, paid-up, irrevocable, worldwide license to publish or reproduce the published form of this written work or allow others to do so, for U.S. Government purposes. The DOE will provide public access to the results of federally sponsored research in accordance with the DOE Public Access Plan.
}
}}

\author{
Thomas Dixon\thanks{Department of Aerospace Engineering, University of Michigan, Ann Arbor, MI, and Optimization and Uncertainty Quantification, Sandia National Laboratories, Albuquerque, NM.}
\and Alex Gorodetsky\thanks{Department of Aerospace Engineering, University of Michigan, Ann Arbor, MI.}
\and John Jakeman\thanks{Optimization and Uncertainty Quantification, Sandia National Laboratories, Albuquerque, NM.}
\and Akil Narayan\thanks{Scientific Computing and Imaging Institute, and Department of Mathematics, University of Utah, UT.}
\and Yiming Xu\thanks{Department of Mathematics, University of Kentucky, KY.
  (\email{yiming.xu@uky.edu}).}}

% Custom SIAM macro to insert headers
\headers{Automating multi-fidelity statistical estimation}{T. Dixon and A. Gorodetsky and J. Jakeman and A. Narayan and Y. Xu}


==> tmp_supplement_header.tex <==
\title{Optimally balancing exploration and exploitation to automate multi-fidelity statistical estimation\thanks{Submitted to the editors on \today.
%\funding{Dixon and Jakeman were supported by the US Department of Energy’s Office of Advanced Scientific Computing Research program. Gorodetsky was supported by the National Nuclear Security Administration’s Advanced Simulation and Computing (ASC) program. Narayan was supported by AFOSR FA9550-20-1-0338 and AFOSR FA9550-23-1-0749. Xu was supported by the University of Kentucky for the start-up funding and the AMS-Simons Travel grant (No.3048116562). Sandia National Laboratories is a multi-mission laboratory managed and operated by National Technology \& Engineering Solutions of Sandia, LLC (NTESS), a wholly owned subsidiary of Honeywell International Inc., for the U.S. Department of Energy’s National Nuclear Security Administration (DOE/NNSA) under contract DE-NA0003525. This written work is authored by an employee of NTESS. The employee, not NTESS, owns the right, title, and interest in and to the written work and is responsible for its contents. Any subjective views or opinions that might be expressed in the written work do not necessarily represent the views of the U.S. Government. The publisher acknowledges that the U.S. Government retains a non-exclusive, paid-up, irrevocable, worldwide license to publish or reproduce the published form of this written work or allow others to do so, for U.S. Government purposes. The DOE will provide public access to the results of federally sponsored research in accordance with the DOE Public Access Plan.
%}
}}

\author{
Thomas Dixon\thanks{Department of Aerospace Engineering, University of Michigan, Ann Arbor, MI, and Optimization and Uncertainty Quantification, Sandia National Laboratories, Albuquerque, NM.}
\and Alex Gorodetsky\thanks{Department of Aerospace Engineering, University of Michigan, Ann Arbor, MI.}
\and John Jakeman\thanks{Optimization and Uncertainty Quantification, Sandia National Laboratories, Albuquerque, NM.}
\and Akil Narayan\thanks{Scientific Computing and Imaging Institute, and Department of Mathematics, University of Utah, UT.}
\and Yiming Xu\thanks{Department of Mathematics, University of Kentucky, KY
  (\email{yiming.xu@uky.edu}).}}

% Custom SIAM macro to insert headers
\headers{Automating multi-fidelity statistical estimation}{T. Dixon and A. Gorodetsky and J. Jakeman and A. Narayan and Y. Xu}

